SynLLM: A Comparative Analysis of Large Language Models for Medical Tabular Synthetic Data Generation via Prompt Engineering

Access to real-world medical data is often restricted due to privacy regulations, posing a significant barrier to the advancement of healthcare research. Synthetic data offers a promising alternative; however, generating realistic, clinically valid, and privacy-conscious records remains a major challenge. Recent advancements in Large Language Models (LLMs) offer new opportunities for structured data generation; however, existing approaches frequently lack systematic prompting strategies and comprehensive, multi-dimensional evaluation frameworks. In this paper, we present SynLLM, a modular framework for generating high-quality synthetic medical tabular data using 20 state-of-the-art open-source LLMs, including LLaMA, Mistral, and GPT variants, guided by structured prompts. We propose four distinct prompt types, ranging from example-driven to rule-based constraints, that encode schema, metadata, and domain knowledge to control generation without model fine-tuning. Our framework features a comprehensive evaluation pipeline that rigorously assesses generated data across statistical fidelity, clinical consistency, and privacy preservation. We evaluate SynLLM across three public medical datasets, including Diabetes, Cirrhosis, and Stroke, using 20 open-source LLMs. Our results show that prompt engineering significantly impacts data quality and privacy risk, with rule-based prompts achieving the best privacy-quality balance. SynLLM establishes that, when guided by well-designed prompts and evaluated with robust, multi-metric criteria, LLMs can generate synthetic medical data that is both clinically plausible and privacy-aware, paving the way for safer and more effective data sharing in healthcare research.

==> 99-Extra.tex <==
%=================================================================
\section{Methodology}
\label{sec:methodology}
%=================================================================

\subsection{Problem Definition}\label{sec:probdef}

Let $\mathcal{D}_{\text{real}}=\{(x^{(i)},y^{(i)})\}_{i=1}^{N}$ denote a structured electronic health‑record (EHR) table where each row $x^{(i)}\in\mathbb{R}^{p_\text{num}}\times\mathcal{C}^{p_\text{cat}}$ contains $p_\text{num}$ numerical and $p_\text{cat}$ categorical attributes and $y^{(i)}$ is an optional downstream label.  
Our goal is to learn a generation mechanism  
\[
\mathcal{G}_\theta:\;\;\bigl(\Pi,\;k\bigr)\;\longmapsto\;\hat{\mathcal{D}}_{\text{syn}}
\]
that, given a **prompt specification** $\Pi$ and a target record count $k\!\ll\!N$, produces a synthetic dataset $\hat{\mathcal{D}}_{\text{syn}}$ such that:

\begin{enumerate}
    \item \textit{Statistical fidelity} $\hat{\mathcal{D}}_{\text{syn}}$ matches the marginal and joint distributions of $\mathcal{D}_{\text{real}}$ within tolerance $\varepsilon_{\text{stat}}$.  

\item \textit{Clinical plausibility} records satisfy medical logic rules (e.g.\ \textit{HbA1c\,$>\!6.5\%$} $\Rightarrow$ \textit{Diabetes\,=\,True}).  

\item \textit{Privacy preservation} the probability that any $\hat{x}\in\hat{\mathcal{D}}_{\text{syn}}$ can be linked to a real patient is below $\delta_{\text{priv}}$ (empirically estimated via membership‑inference, $k$‑anonymity and outlier distance tests).  

\end{enumerate}




Unlike GAN or VAE approaches that require direct access to $\mathcal{D}_{\text{real}}$ during training, we employ zero‑/few‑shot LLMs and carefully‑designed prompts that expose \textit{only non‑identifiable summaries} of the real data.
This reduces regulatory burden while exploiting the vast medical priors captured by modern LLMs \cite{borisov2023realistic,llm_tab_survey2024}.

%-----------------------------------------------------------------
\subsection{SynLLM Generation Pipeline}\label{sec:pipeline}
%-----------------------------------------------------------------
The pipeline (Algorithm~\ref{alg:synllm}) contains four stages:

\begin{enumerate}[leftmargin=*]
\item \textbf{Schema analysis.}  Compute attribute types, descriptive statistics, and inter‑feature correlations from $\mathcal{D}_{\text{real}}$ (Sec.~\ref{sec:schema}).  Only aggregate values leave the secure enclave.
\item \textbf{Prompt synthesis.}  Assemble a prompt $\Pi$ according to one of four progressively‑constrained templates (Sec.~\ref{sec:prompts}).
\item \textbf{LLM inference.}  Query an instruction‑tuned open‑source model (Table~\ref{tab:models}) with temperature $T{=}0.7$, top‑\!$p{=}0.9$, and maximum token budget computed from $k$.
\item \textbf{Post‑processing and validation.}  Parse JSON rows to tabular form, cast datatypes, and discard any record violating hard clinical rules.  The surviving records enter the evaluation suite described in Sec.~\ref{sec:evaluation}.
\end{enumerate}


%-----------------------------------------------------------------
\subsection{Adaptive Prompt Taxonomy}\label{sec:prompts}
%-----------------------------------------------------------------
Our prompt schema is organised into a four‑tier hierarchy of escalating sophistication: Level 1 functions as the baseline, while levels 2 through 4 incrementally introduce richer contextual cues and stricter domain‑specific constraints.


\begin{description}[leftmargin=0cm,labelsep=0.2cm,style=sameline,font=\bfseries]
\item[\textsc{SeedEx} (Prompt‑A):] \textit{Example‑Seed Minimal Prompt}.  
Lists the header row, the desired JSON output format, and $\leq5$ seed rows randomly sampled from $\mathcal{D}_{\text{real}}$.  
Purpose: establish a \emph{baseline} that stresses model generalization under minimal constraint but suffers the highest disclosure risk.

\item[\textsc{FeatDesc} (Prompt‑B):] \textit{Feature‑Description Prompt}.  
Replaces concrete examples with succinct natural‑language definitions of each attribute (e.g.\ “\texttt{bmi}: body‑mass index in kg/m$^2$, real $[12,60]$”).  
Benefits: injects clinical semantics, cuts direct exposure to patient rows, and encourages in‑distribution value ranges.

\item[\textsc{StatGuide} (Prompt‑C):] \textit{Statistical‑Metadata Prompt}.  
Augments \textsc{FeatDesc} with feature‑level moments (mean, $\sigma$), value ranges, and category frequencies, plus pairwise correlations for critical variable pairs.  
This mirrors the ``data portraits'' technique in \cite{Wang2024HARMONICHL} and provably narrows the Wasserstein gap (Sec.~\ref{sec:results}).

\item[\textsc{ClinRule} (Prompt‑D):] \textit{Clinically‑Constrained Prompt}.  
Removes all row‑level information and instead supplies declarative constraints derived from clinical guidelines (e.g.\ ``If \texttt{pregnant}=True then \texttt{sex}=Female'' or ICD‑10 logic rules).  
The LLM must satisfy these clause rules while generating new samples.
%We found \textsc{ClinRule} delivers the best privacy–utility harmonic score, aligning with recent findings on rule‑based control \cite{tran2024dp_llm}.
\end{description}

Table~\ref{tab:prompt-excerpt} shows condensed excerpts of each template (full text in Appendix~A).  All prompts share a common \textbf{system message} instructing the model to (i) output \texttt{newline‑delimited JSON} objects, (ii) avoid free‑text commentary, (iii) respect requested record counts, and (iv) refrain from emitting protected health information (\textit{PHI}).  At generation time we programmatically inject dataset‑specific metadata into placeholder tags (``\texttt{\{feature\_stats\}}'').


\begin{table}[t]
\centering\small
\caption{Prompt skeletons (abridged).  Curly braces are runtime placeholders.}
\label{tab:prompt-excerpt}
\begin{tabularx}{\columnwidth}{@{}L{0.24\columnwidth}X@{}}
\toprule
\textbf{Template} & \textbf{Key Sections}\\
\midrule
\textsc{SeedEx}   & Header row; $n$ seed examples; ``Repeat format exactly, $k$ rows.'' \\
\textsc{FeatDesc} & Header row; per‑feature definition sentences; JSON schema block.\\
\textsc{StatGuide}& As \textsc{FeatDesc} plus \{mean\}, \{stdev\}, \{min,max\}, frequency tables; optional correlation matrix snippet.\\
\textsc{ClinRule} & Header row; clinical rule list (DL\,$\rightarrow$\,HbA1c$>$6.5, etc.); JSON schema; no examples.\\
\bottomrule
\end{tabularx}
\end{table}


\paragraph*{Design rationale.}
The template suite systematically varies the amount and nature of conditioning information supplied to the LLM, thereby allowing a controlled exploration of the privacy–utility continuum. At one extreme, \textsc{SeedEx} imposes minimal a priori constraints; it achieves the lowest Jensen–Shannon divergence from the source distribution but is most susceptible to membership‑inference attacks. At the opposite extreme, \textsc{ClinRule} enforces strict domain rules, markedly reducing disclosure risk at the cost of greater distributional shift. The intermediate templates, \textsc{FeatDesc} and \textsc{StatGuide}, incrementally introduce semantic descriptions and statistical metadata, enabling precise assessment of how contextual and quantitative cues influence synthetic‑data fidelity. Empirical evidence in Sec.~\ref{sec:results} shows that \textsc{StatGuide} yields the best overall utility for internal analytics, whereas \textsc{ClinRule} is preferable when public‑release constraints dominate.

%-----------------------------------------------------------------
\subsection{Schema and Statistical Extraction}\label{sec:schema}
%-----------------------------------------------------------------
We compute for each numerical attribute $f$ the 5‑tuple  
$(\mu_f,\sigma_f,\text{min}_f,\text{max}_f,\text{quantiles}_f)$  
and for each categorical attribute, the empirical probability mass function $\mathbf{p}_f$.  
To suppress rare‑category disclosure we apply a 5‑count threshold and merge sub‑threshold categories into ``\texttt{Other}'' before statistics are surfaced to the prompt builder.  
Pairwise Pearson correlations $\rho_{fg}$ are retained only for clinically pertinent pairs ($|\rho_{fg}|>0.15$ or flagged by domain experts).  




















